DexFuture: Hierarchical Future-State Visuomotor Targeting for Bimanual Dexterous Tool Use

Bimanual dexterous tool use remains challenging for robots due to high-dimensional hand configurations and complex hand-tool-object dynamics and contact. Most existing control policies depend on future configuration references provided from demonstrations, while future action-conditioned world models require slow online planning over high-dimensional action sequences. A significant challenge is generating a dynamically consistent future reference trajectory without relying on privileged states from demonstrations or slow counterfactual planning. We propose DexFuture, a hierarchical system that couples a high-level Future-State Visuomotor Target Predictor with a low-level Target-Conditioned Structured Dexterous Policy. Conditioned on egocentric RGB, proprioceptive and geometric history, the high-level predictor constructs structured hand-tool-object visuomotor embeddings and uses a horizon-conditioned transformer to generate a multi-step future target trajectory. Then, the low-level policy tracks them with a target-conditioned per-link transformer. This hierarchy decouples coarse future reference generation from fine-grained action control, and slow long-horizon semantic prediction from high-frequency execution. On OakInk2 bimanual tool-use tasks, DexFuture achieves 90% of the privileged-oracle performance, compared to 7% for a no-reference policy. DexFuture operates at 60 Hz, approximately 250 times faster than DexWM-style Cross-Entropy Method (CEM) planning with a future action-conditioned world model.

==> dexfuture/sec/backup.tex <==
Bimanual dexterous tool use remains a formidable challenge in robotics due to high-dimensional hand control, coordinated multi-contact interactions, and complex hand--tool--object dynamics. Recent target-conditioned dexterous policies make such tasks more tractable by tracking future targets extracted from demonstration trajectories. However, these targets contain privileged future hand, tool, and object states, and are unavailable at deployment. Action-conditioned world models provide another route through online planning, but require expensive optimization over high-dimensional future actions, making them impractical for high-frequency contact-rich dexterous control. We propose \textbf{DexFuture}, a hierarchical future-state visuomotor targeting framework that removes the need for privileged future demonstration targets. DexFuture uses a high-level Future-State Visuomotor Target Predictor to infer a coarse multi-step target window from causal egocentric RGB and proprioceptive/geometric history. A low-level target-conditioned structured dexterous policy then tracks the predicted and interpolated targets at every simulator step to execute fast bimanual actions. This hierarchy separates future-state targeting from action-level control, and slow semantic prediction from high-frequency execution. On challenging OakInk2 bimanual tool-use tasks, DexFuture recovers the benefit of target-conditioned control without privileged future targets, achieving $59.69\%$ average success rate compared with $7.36\%$ for the no-target policy and about $90\%$ of the privileged oracle. DexFuture also executes at $60$Hz, approximately $250\times$ faster than CEM-based action-conditioned planning in our setup. Our results show that predicted future-state targets provide an efficient and practical interface between visuomotor perception and dexterous control.




We propose DexFuture, a hierarchical system that couples a high-level Future-State Visuomotor Predictor with a low-level Physically-Grounded Dexterous Policy. The predictor converts RGB observations and proprioception into structured future-state targets, which replace privileged demonstration targets during inference, while the policy executes contact-rich bimanual tool-use manipulation through physically-grounded attention.


DexFuture, A hierarchical visuomotor framework that couples a slow predictive visual target generator with a fast physically-grounded dexterous control policy. .




During DexFuture execution, the same slot is filled with the target predicted by Eq.~\eqref{eq:target_decoder}. This isolates the key question studied in this paper: whether the benefit of target-conditioned dexterous control can be preserved when future targets are inferred from visuomotor history rather than provided by privileged demonstration state.

While the high-level visuomotor predictor predicts coarser guidance, our low-level has the ability to correct the action with the noisy guidance input.

We use artimano hands


\begin{wraptable}[13]{r}{0.50\textwidth}
\vspace{-0.8em}
\centering
\caption{\textbf{Future-state target prediction accuracy.}
We report 3D error, UV error, and PCK within 5/10 pixels.}
\label{tab:predictor_eval}
\vspace{-0.5em}
\footnotesize
\setlength{\tabcolsep}{2pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccc@{}}
\toprule
\textbf{Task ID} &
\textbf{3D} $\downarrow$ &
\textbf{UV} $\downarrow$ &
\textbf{PCK@5} $\uparrow$ &
\textbf{PCK@10} $\uparrow$ \\
\midrule
083f7@0  & 1.47 & 3.32  & 79.56 & 98.37 \\
9fc3e@0  & 0.87 & 2.56  & 91.34 & 99.78 \\
598a5@0  & 1.31 & 2.73  & 90.24 & 97.82 \\
1292e@0  & 2.31 & 6.91  & 38.49 & 80.02 \\
b4a4e@1  & 3.17 & 14.49 & 13.92 & 41.45 \\
817fb@0  & 4.54 & 8.74  & 19.33 & 68.27 \\
e1fa67@0 & 5.54 & 25.58 & 7.98  & 32.93 \\
9bb17@5  & 4.50 & 12.86 & 22.31 & 54.15 \\
cde36@1  & 1.65 & 5.41  & 76.93 & 95.76 \\
\bottomrule
\end{tabular*}
\vspace{-0.9em}
\end{wraptable}


\begin{wraptable}[12]{r}{0.50\linewidth}
\vspace{-1.0em}
\centering
\caption{\textbf{Ablation of future prediction horizon.}
We compare different future horizon schedules using 3D error, UV error, and PCK within 5/10 pixels.}
\label{tab:horizon_ablation}
\vspace{-0.5em}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Task ID} &
\textbf{3D} $\downarrow$ &
\textbf{UV} $\downarrow$ &
\textbf{PCK@5} $\uparrow$ &
\textbf{PCK@10} $\uparrow$ \\
\midrule
083f7@0\_h24  & 1.66 & 4.05 & 71.87 & 97.54 \\
083f7@0\_h16  & 1.47 & 3.32 & 79.56 & 98.37 \\
083f7@0\_h8   & 1.19 & 3.68 & 76.99 & 96.34 \\
9fc3e@0\_h24  & 1.11 & 2.95 & 86.66 & 99.27 \\
9fc3e@0\_h16  & 0.87 & 2.56 & 91.34 & 99.78 \\
9fc3e@0\_h8   & 0.84 & 2.46 & 92.15 & 99.72 \\
598a5@0\_h24  & 1.77 & 3.97 & 73.56 & 97.46 \\
598a5@0\_h16  & 1.31 & 2.73 & 90.24 & 97.82 \\
598a5@0\_h8   & 1.38 & 2.86 & 89.72 & 97.40 \\
\bottomrule
\end{tabular}}
\vspace{-1.0em}
\end{wraptable}



\iffalse
\begin{table}[htbp]
\centering
\begin{minipage}{0.5\linewidth}
\centering
\caption{\textbf{Quantitative results on bimanual tool-use tasks of Oakink2 dataset \cite{oakink2}.} Link 3D Error (cm), Percentage of correct key points, Link UV Error (pix), link\_pck\_5px (\%), link\_pck\_10px (\%)}
\label{table:physgraph_results}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Task ID}  & \textbf{3D} $\uparrow$ & \textbf{UV} $\downarrow$ & \textbf{pck\_5px} $\uparrow$ & \textbf{pck\_10px} $\uparrow$ \\ 
\midrule
{083f7@0\_h24}   & 1.66 & 4.05 & 71.87 & 97.54 \\
{083f7@0\_h16}   & 1.47 & 3.32 & 79.56 & 98.37 \\
{083f7@0\_h8}   & 1.19 & 3.68 & 76.99 & 96.34 \\
{9fc3e@0\_h24}   & 1.11 & 2.95 & 86.66 & 99.27 \\
{9fc3e@0\_h16}   & 0.87 & 2.56 & 91.34 & 99.78 \\
{9fc3e@0\_h8}   & 0.84 & 2.46 & 92.15 & 99.72  \\
{598a5@0\_h24}  & 1.77 & 3.97 & 73.56 & 97.46 \\
{598a5@0\_h16}  & 1.31 & 2.73 & 90.24 & 97.82 \\
{598a5@0\_h8}  & 1.38 & 2.86 & 89.72 & 97.40 \\
\bottomrule
\end{tabular}
\label{tab:horizon_ablation}
}
\end{minipage}
\end{table}
\fi

==> dexfuture/sec/conclusions.tex <==
\section{Conclusion}
\label{sec:conclusion}
We presented \textbf{DexFuture}, a hierarchical future-state visuomotor targeting framework for bimanual dexterous tool use. DexFuture removes the need for privileged future demonstration targets by predicting future targets conditioned on RGB and proprioceptive/geometric history, while a low-level structured policy executes high-frequency contact-rich actions. This design preserves the benefit of target-conditioned dexterous control without requiring future demonstration states or slow online action-sequence planning. Experiments on challenging tool-use tasks show that DexFuture mostly retains the performance of privileged baselines, strongly outperforms no-target control, and runs substantially faster than counterfactual planning.

==> dexfuture/sec/dexfuture.tex <==
\section{Method}

\subsection{Hierarchical Problem Formulation}

\begin{figure*}[!t]
  \centering
  \includegraphics[width=\textwidth]{dexfuture/figures/pipeline.pdf}
\caption{
    \textbf{DexFuture overview.}
    DexFuture is a hierarchical system that separates bimanual dexterous manipulation into slow future target generation and fast action-level control.
    \textbf{A.} Given recent egocentric RGB observations and proprioceptive/geometric states, we construct structured visuomotor tokens instead of passing dense image patches to the predictor. Hand-link embeddings are obtained by projecting each link into the image and cross-attending to local visual patches, while tool/object embeddings are built by anchor-aligned visual sampling and entity-state/geometry embeddings.
    \textbf{B.} The Horizon-Conditioned Target Transformer takes the structured embedding history as memory and predicts sparse future structured embeddings at horizons $\mathcal{H}=\{0,2,4,\ldots,16\}$. Future embeddings are first initialized from the latest observed state and modulated with learned future-index embeddings and Fourier horizon encodings, then refined via self-attention and cross-attention to the visuomotor history using AdaLN-Zero transformer blocks. The predicted embeddings are decoded into auxiliary geometric states for supervision, and a $900$-D future target used by the low-level policy.
    \textbf{C.} The target-conditioned structured dexterous policy consumes the current state and the predicted target, tokenizes the bimanual hand-tool-object system into per-link and scene embeddings, and outputs a bimanual action distribution through a transformer encoder and policy head.
    \textbf{D.} During receding-horizon execution, a single forward pass of the visuomotor predictor produces a target trajectory over multiple time steps. Intermediate targets are linearly interpolated to allow high-frequency feedback control. The predictor is trained with supervised latent, state, and target losses, while the policy is trained with PPO against a tracking reward.
}
    \vspace{-5mm}
    \label{fig:policy_overview}
\end{figure*}



%We consider bimanual dexterous manipulation, where two multi-fingered hands coordinate contacts with a tool and an object under complex rigid-body dynamics. Recent dexterous manipulation policies make learning tractable by conditioning the policy on future targets extracted from the demonstration trajectory \cite{dexmachina, dextrack, omnigrasp, maniptrans, physgraph}. 

%The absence of future target demonstration as the input always lead to failed policy training for High-DoF dexterous hands in bimanual challenging tasks. The target reference contains desired future wrist motion, hand-link motion, object pose, contact-related fingertip information, and shape-level task cues. However, it is also privileged. At inference time, the robot observes the current scene and proprioception, but does not have access to the future demonstration state of the hands, tool, object. Thus, the practical bottleneck is not only learning a strong dexterous controller, but also obtaining the future target that control policies require.

%We propose \emph{DexFuture} to address this bottleneck through a hierarchical future-targeting formulation. Given a short history of RGB observations and proprioceptive/geometric cues,


Figure \ref{fig:policy_overview} shows an overview of DexFuture. Let $s_t$ be the current robot-object state, $a_t$ be the bimanual hand action, and $g^{\mathrm{demo}}_{t+h}$ be a future demonstration target with horizon $h$. A target-conditioned dexterous policy can be written as
%
\begin{equation}
a_t \sim \pi_{\phi}(\cdot \mid s_t, g^{\mathrm{demo}}_{t+h}).
\label{eq:demo_target_policy}
\end{equation}
%
The target $g^{\mathrm{demo}}_{t+h}$ provides future reference for high-DoF dexterous control but it is privileged: at inference, the robot observes the current scene and proprioception, not the future demonstration state of the hands, tool, or object. 
%Therefore, we propose \textbf{DexFuture} to 
Thus, our main objective is to predict future targets from the visuomotor history. We assume access to a history of $K$ RGB observations and proprioceptive/geometric cues:
%
\begin{equation}\label{eq:obs_history}
\mathcal{O}_{t-K:t}=\{I_{\tau},p_{\tau}\}_{\tau=t-K}^{t},
\end{equation}
%

where $I_{\tau}$ is the RGB observation and $p_{\tau}$ denotes structured proprioceptive and available geometric cues. Given this visuomotor history, DexFuture predicts future targets up to horizon $h$ as:
%\NA{It would help to show a figure visualizing the setup -- observations, proprioceptive cues, geometric cues.}, 
%we learn a predictor that estimates a sequence of future targets over a sparse horizon set $\mathcal{H}=\{h_1,\ldots,h_M\}$:
%\NA{I am not sure what a "sparse horizon set" is. Is it really needed? Can we just predict $\hat{g}_{t+h}$? Why is the notation below $\hat{\mathbf{g}}_{t:t+H}$ different from the target notation $g^{\mathrm{demo}}_{t+h}$? Are we predicting a different thing? I see below that we interpolate $\tilde{g}$ from $\hat{\bfg}$ but we should simplify the presentation of this here. First explain that we predict $\hat{g}_{t+h}$ instead of using $g_{t+h}$ directly and then later, you can get into the details that this uses a composition of Interp and $F_{\theta}$.}
%
\begin{equation}\label{eq:future_target_prediction}
\hat{g}_{t+h}=F_{\theta}(\mathcal{O}_{t-K:t};\mathcal{H}).
\end{equation}
%
Here, $F_{\theta}$ is our \emph{Future-State Visuomotor Target Predictor}, and $\hat{g}_{t+h}$ is the predicted target trajectory, which has the same representation as the demonstrations $g^{\mathrm{demo}}_{t+h}$, but is inferred from observation history rather than being given from demonstrations. In practice, we predict targets up to a finite horizon $\mathcal{H}$ with coarser intervals, such as $\mathcal{H}=\{0,2,\ldots,16\}$, and use interpolation for intermediate control steps. The low-level policy then executes
\begin{equation}
a_{t+\delta}
\sim
\pi_{\phi}(\cdot \mid s_{t+\delta}, \tilde{g}_{t+\delta}),
\qquad
\tilde{g}_{t+\delta}
=
\mathrm{Interp}\left(\{\hat{g}_{t+h}\}_{h\in\mathcal{H}},\delta\right),
\label{eq:pred_target_policy}
\end{equation}
%where $\tilde{g}_{t+\delta}$ is the target used by the policy at an intermediate future control step $t+\delta$, obtained by interpolating the sparse predicted targets.

%This formulation creates two complementary hierarchies. First, DexFuture separates \emph{future state targeting} from \emph{action-level control}: the predictor is high-level action-free and estimates where the manipulation should progress in future state space, while the policy handles low-level high-frequency motor commands and contact correction. Second, DexFuture separates \emph{semantic prediction time} from \emph{control time}: one predictor update summarizes a short observation history and produces a target window spanning multiple low-level policy steps.

%This design is different from action-conditioned world-model planning. Action-conditioned models are well-suited for counterfactual rollouts, but using them for control requires optimizing over many candidate future action sequences. For high-DoF dexterous hands, this planning loop can be prohibitively expensive. Moreover, in a target-conditioned policy pipeline, future actions depend on predicted future targets, while action-conditioned prediction would require future actions as input. DexFuture avoids this circular dependency by predicting the future target interface directly from visuomotor history and delegating physical execution to the dexterous policy. 

%Our main contribution is therefore a hierarchical target-generation framework that removes the reliance on privileged future demonstration targets while preserving the benefits of target-conditioned dexterous control. We next describe how DexFuture constructs structured visuomotor tokens, predicts sparse-horizon future targets, and executes them with a structured dexterous policy. We provide the step-by-step details and pseudo-code of our method in the supplementary material.


This formulation yields a compact hierarchy: $F_\theta$ predicts an action-free future target window over multiple low-level steps, while $\pi_\phi$ executes high-frequency actions using the interpolated targets. Unlike action-conditioned world-model planning, the predictor does not require candidate future actions as input, avoiding online action-sequence optimization and the circular dependency between future actions and future targets. The following sections describe how DexFuture constructs structured visuomotor embeddings, predicts sparse-horizon future targets, and executes them with the target-conditioned policy. We also provide more details and pseudo-code in the \emph{supplementary}.

\subsection{Future-State Visuomotor Target Predictor}

%The \emph{Future-State Visuomotor Target Predictor} is designed around the interface required by dexterous control. Instead of generating future pixels \cite{dexwm} or directly predicting actions \cite{lat_act_diff}, it predicts a future target representation that can be consumed by a downstream target-conditioned policy. This choice is motivated by the structure of dexterous manipulation: successful execution depends on higher-level future hand-object geometry, fingertip relations, object motion, and task-shape cues, while precise contact stabilization is better handled by a lower-level high-frequency controller.

%A naive design would encode the entire image into a global visual feature and regress the target vector directly. However, bimanual dexterous manipulation is inherently local and structured. Fingertip contacts occur at specific links, tool interaction depends on local hand-object geometry, and the controller itself reasons over per-link state. We therefore first convert RGB-state history into structured per-link visuomotor tokens.

The \emph{Future-State Visuomotor Target Predictor} predicts the target states tracked by the low-level policy, rather than future pixels or actions. This follows the DexFuture hierarchy: the predictor provides coarse future hand-tool-object state guidance, while fine contact-rich control is handled by the low-level policy.

The target states exhibit a kinematic structure that allows decomposition into the hand, tool and the object. 
Therefore, it is unnecessary to use \emph{all} visual patches from the images to encode the visuomotor history, which may also be poorly aligned with the output.    
Instead, we propose a more structured embedding that exploits the physical relationship between the visual and proprioceptive information to extract only the relevant visual information.

% Therefore, directly feeding dense visual patch tokens 
% Since this target interface is structured\BL{Unclear what structured means}, directly feeding dense visual patch tokens into the multi-horizon transformer is both computationally expensive and poorly aligned with the hand-link, tool, and object components of the output. 
% Therefore, we use proprioceptive/geometric states to form structured physical queries, and extract only the relevant local visual evidence needed to build compact visuomotor tokens.
For each observed frame, a frozen visual encoder extracts patch-level image features. Each hand link is projected into the image, and we collect the local visual neighborhood around the projected link. The query vector for the projected link, constructed from its identity, 3D position, and 2D projection, only attends to this local visual neighborhood to produce a link-level visuomotor embedding. Tool and object embeddings are constructed from their current state, geometry, type, projected center, and visual features. Together, these embeddings form a compact physical representation as
\begin{equation}
Z_t =
\{z^{\mathrm{hand}}_{t,i}\}_{i=1}^{N_h}
\cup
\{z^{\mathrm{tool}}_t,z^{\mathrm{obj}}_t\},
\label{eq:structured_tokens}
\end{equation}
where $Z_t$ is the structured embeddings at time $t$, $N_h$ is the number of hand-link tokens, $z^{\mathrm{hand}}_{t,i}$ is the embedding for hand link $i$, and $z^{\mathrm{tool}}_t,z^{\mathrm{obj}}_t$ are the tool and object embeddings. 
%\BL{Decide on token vs embedding and use consistently}

\paragraph{Horizon-Conditioned Target Transformer.}
Given the structured history $Z_{t-K:t}$, DexFuture predicts future targets at sparse timesteps over a horizon. The observed history embeddings serve as memory. Future query  vectors %\BL{this could be query vectors} 
are initialized from the latest visuomotor embeddings %\BL{this could be visuomotor embedding, or sth like that} 
$Z_t$, since future manipulation states are naturally predicted as transformations of the current hand-tool-object state. Each future timestep $h\in\mathcal{H}$ receives a horizon embedding, allowing the shared transformer to specialize its prediction for near and distant futures. We write this prediction compactly as
\begin{equation}
\hat{Z}_{t+h}=T_{\theta}(Z_t, Z_{t-K:t}, h),
\qquad h\in\mathcal{H},
\label{eq:horizon_transformer}
\end{equation}
where $T_{\theta}$ is the horizon-conditioned transformer and $\hat{Z}_{t+h}$ is the predicted structured embeddings at timestep $h$. Architecturally, this module uses adaptive layer-normalization conditioning from conditional diffusion transformer (CDiT) blocks \cite{cdit}. Horizon information modulates transformer updates through adaptive normalization and gated residual paths. However, unlike diffusion models, we remove the iterative denoising in DexFuture to directly regress sparse future targets for fast inference. The predicted future embeddings are decoded into auxiliary physical states and the target representation used by the dexterous policy:
\begin{equation}
\hat{g}_{t+h}=D_{\theta}(\hat{Z}_{t+h}),
\qquad h\in\mathcal{H},
\label{eq:target_decoder}
\end{equation}
where $D_{\theta}$ is the target decoder. The decoded target has the same layout as the demonstration target used by the policy so that the policy interface remains the same. During training, $F_{\theta}$ is supervised from demonstration using a future imitation target loss and an auxiliary future embedding loss: %\BL{again, embedding? can we call these imitation losses?}
\begin{equation}
\mathcal{L}_{\mathrm{pred}}
=
\lambda_{\mathrm{state}}\mathcal{L}_{\mathrm{state}}
+
\lambda_{\mathrm{target}}\mathcal{L}_{\mathrm{target}}.
\label{eq:prediction_loss}
\end{equation}
Here, $\mathcal{L}_{\mathrm{state}}$ supervises future hand-link, tool, and object states, while $\mathcal{L}_{\mathrm{target}}$ supervises the decoded policy target. The exact target decomposition is described in the \textbf{supplementary material}.

\subsection{Target-Conditioned Structured Dexterous Policy}

DexFuture can be paired with any low-level dexterous controller that consumes a structured future target. In our experiments, we instantiate the controller as a target-conditioned per-link transformer policy, inspired from \cite{physgraph}. The policy tokenizes the current bimanual hand-tool-object state and the target into hand-link tokens, scene tokens, and a policy token. A transformer encoder processes these tokens, and the final policy token parameterizes a Gaussian action distribution,
\begin{equation}
a_t\sim\mathcal{N}\left(\mu_{\phi}(s_t,\tilde{g}_t),\Sigma_{\phi}\right),
\label{eq:policy_distribution}
\end{equation}
where $\mu_{\phi}$ is the action mean and $\Sigma_{\phi}$ is a learned diagonal covariance.

The policy is trained with PPO \cite{PPO} using tracking rewards against demonstration trajectories. The reward includes tracking terms for wrist pose, hand-link/fingertip positions, object pose, object velocity, object angular velocity, and energy regularization. During privileged baseline evaluation, 
%\BL{not sure what oracle evaluation means here. Also, we are saying we do not use demonstration target. Can we remove this sentence?}, 
the target is replaced with the demonstration target. 

\subsection{Hierarchical Receding-Horizon Execution}
At inference time, DexFuture executes the system hierarchy in a receding-horizon manner. At refresh time $t_j$, the predictor observes the recent history and produces a sparse future target sequence. For each low-level control step $t_j+\delta$ before the next refresh, the policy receives an interpolated target and computes an action from the current state:
\begin{equation}
\hat{\mathbf{g}}_{t_j:t_j+H}
=
F_{\theta}(\mathcal{O}_{t_j-K:t_j};\mathcal{H}),
\qquad
a_{t_j+\delta}
\sim
\pi_{\phi}(\cdot \mid s_{t_j+\delta},
\mathrm{Interp}(\hat{\mathbf{g}}_{t_j:t_j+H},\delta)).
\label{eq:receding_horizon_execution}
\end{equation}
This execution scheme enables the predictor to operate at a slower timescale while the policy remains reactive at the control timescale. The predicted targets need not be physically exact action-level rollouts. Instead, they provide coarser future state guidance, while the low-level policy performs finer contact-level correction and action execution.

==> dexfuture/sec/experiments.tex <==
\section{Experimental Results}
\label{sec:result}

\begin{table*}[t]
\centering
\caption{\textbf{Quantitative results on bimanual tool-use tasks of Oakink2 dataset \cite{oakink2}.} SR: Success Rate; E\_t: Tool \& Object Translation Error; E\_j: Hand Joint Error; E\_ft: Fingertip Error.}
\label{table:physgraph_results}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lll cccc}
\toprule
\textbf{Task ID}  & \textbf{Task / Tool (R) / Object (L)} & \textbf{Methods} & \textbf{SR (\%)} $\uparrow$ & \textbf{E\_t (cm)} $\downarrow$ & \textbf{E\_j (cm)} $\downarrow$ & \textbf{E\_ft (cm)} $\downarrow$ \\ \midrule

\multirow{3}{*}{083f7@0}  & \multirow{3}{*}{cut / chop knife / bread} & Maniptrans (GT target) & 55.69 & 1.31 & 2.42 & 2.01 \\
 & & PhysGraph (GT target) & \textbf{90.05} & \textbf{0.69} & 2.17 & \textbf{1.42} \\
 & & PhysGraph (No target) & 4.16 & 1.87 & 3.11 & 2.68 \\
 & & DexFuture (Pred target) & 83.49 & 1.06 & \textbf{2.08} & 2.04 \\ \hline
 
 \multirow{3}{*}{9fc3e@0}  & \multirow{3}{*}{cut / fruit knife / apple} & Maniptrans (GT target) & 70.58 & 0.84 & 2.99 & \textbf{1.97} \\
 & & PhysGraph (GT target) & 87.87 & 0.98 & 2.04 & 2.17 \\ 
 & & PhysGraph (No target) & 20.5 & 1.42 & 2.34 & 2.45 \\
 & & DexFuture (Pred target) & \textbf{89.79} & \textbf{0.61} & \textbf{2.03} & 2.40 \\ \hline


\multirow{3}{*}{1292e@0} & \multirow{3}{*}{pour / mug / mug} & Maniptrans (GT target) & 45.60 & 6.78 & 3.50 & \textbf{3.35} \\
 & & PhysGraph (GT target) & \textbf{49.77} & \textbf{5.93} & \textbf{3.07} & 4.33 \\
 & & PhysGraph (No target) & 1.82 & 8.37 & 4.13 & 4.48 \\
 & & DexFuture (Pred target) & 41.05 & 7.27 & 3.82 & 3.85 \\ \hline


\multirow{3}{*}{817fb@0} & \multirow{3}{*}{wipe / big brush / whiteboard} & Maniptrans (GT target) & 50.05 & 1.55 & 2.17 & 2.24 \\
 & & PhysGraph (GT target) & \textbf{62.24} & \textbf{1.33} & \textbf{1.54} & \textbf{1.86} \\
 & & PhysGraph (No target) & 8.99 & 2.77 & 2.68 & 2.58 \\
 & & DexFuture (Pred target) & 56.96 & 1.50 & 2.42 & 2.43 \\ \hline

 \multirow{3}{*}{fc88d@0} & \multirow{3}{*}{wipe / small brush/ whiteboard} & Maniptrans (GT target) & 71.21 & 1.21 & \textbf{2.44} & 1.79 \\
 & & PhysGraph (GT target) & \textbf{80.65} & \textbf{1.11} & 2.49 & \textbf{1.50} \\
 & & PhysGraph (No target) & 4.87 & 2.23 & 3.72 & 3.04 \\
 & & DexFuture (Pred target) & 67.17 & 1.25 & 3.02 & 1.70 \\ \hline

\multirow{3}{*}{e1fa6@0} & \multirow{3}{*}{shear / scissors / paper} & Maniptrans (GT target) & 15.16 & \textbf{1.18} & 3.31 & 2.25 \\
 & & PhysGraph (GT target) & \textbf{35.84} & 1.35 & \textbf{2.52} & \textbf{1.83} \\
 & & PhysGraph (No target) & 0.00 & 1.78 & 3.70 & 2.68 \\
 & & DexFuture (Pred target) & 30.69 & 1.62 & 2.97 & 1.92 \\ \hline

 \multirow{3}{*}{9bb17@5} & \multirow{3}{*}{shear / scissors / paper} & Maniptrans (GT target) & 51.68 & 1.93 & \textbf{2.26} & 2.86 \\
 & & PhysGraph (GT target) & \textbf{59.21} & \textbf{1.90} & 3.12 & \textbf{2.70} \\
 & & PhysGraph (No target) & 11.18 & 3.85 & 3.81 & 3.93 \\
 & & DexFuture (Pred target) & 48.66 & 2.49 & 2.73 & 2.90 \\


\bottomrule
\vspace{-3mm}
\label{tab:policy}
\end{tabular}}
\end{table*}



\subsection{Experimental Setup}

We evaluate DexFuture on challenging bimanual dexterous tool-use tasks from OakInk2 \cite{oakink2}, including cutting, pouring, wiping, shearing, and stirring. Each task requires coordinated interaction among two dexterous hands, a tool, and an object. We compare DexFuture against two strong target-conditioned dexterous policy baselines: ManipTrans \cite{maniptrans} and PhysGraph \cite{physgraph}. For these baselines, the target is provided from the \emph{ground-truth} future demonstration state. We also include a no-target variant of the PhysGraph policy, which removes the future target input and tests whether the policy can perform the task from the current state alone. We report success rate (SR), tool/object translation error $E_t$, hand joint error $E_j$, and fingertip error $E_{ft}$. Higher SR is better, while lower tracking errors are better. Implementation details, reward terms, training hyperparameters, evaluation metrics definition, and results of more tasks are provided in the \textbf{supplementary}.


\subsection{Policy Evaluation with Predicted Future Targets}

The core question of policy evaluation is whether DexFuture can retain the benefit of target-conditioned dexterous control without using privileged future demonstration targets at inference. Table~\ref{tab:policy} summarizes the policy performance. The ``no-target'' policy shows that simply removing the future target makes high-DoF dexterous tool use nearly infeasible, while DexFuture recovers a strong target signal from visuomotor history.

Compared with the privileged structured-policy, DexFuture achieves about $90\%$ of the average success rate of privileged baselines ($59.69\%$ vs. $66.52\%$), despite using predicted targets instead of ground-truth future demonstration targets. On the fruit-knife cutting task, DexFuture even slightly outperforms the privileged baseline in success rate ($89.79\%$ vs. $87.87\%$) and tool/object translation error ($0.61$cm vs. $0.98$cm). On the bread-cutting, whiteboard-wiping, and paper-shearing tasks, DexFuture remains close to the privileged baseline while significantly outperforming the no-target variant. These results support our main claim: future target guidance is essential for dexterous tool use, but it does not have to be provided by online privileged demonstration state.

%DexFuture is naturally weaker than the oracle on challenging tasks where long-horizon contact evolution is difficult to infer from short visual history, such as shearing with scissors. The prediction errors in the future target can stream into poorer low-level contact in the policy. However, our predicted-target policy remains substantially better than removing the target entirely, indicating that even imperfect future-state guidance is highly valuable for bimanual dexterous control.



\subsection{Future-State Visuomotor Target Prediction}
\label{sec:exp:predictor}

\begin{wraptable}[12]{r}{0.50\textwidth}
\vspace{-0.8em}
\centering
\caption{\textbf{Future-state target prediction accuracy.}
We report 3D error, UV error, and PCK within 5/10 pixels.}
\label{tab:predictor_eval}
\vspace{-0.5em}
\footnotesize
\setlength{\tabcolsep}{2pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccc@{}}
\toprule
\textbf{Task ID} &
\textbf{3D} $\downarrow$ &
\textbf{UV} $\downarrow$ &
\textbf{PCK@5} $\uparrow$ &
\textbf{PCK@10} $\uparrow$ \\
\midrule
083f7@0  & 1.47 & 3.32  & 79.56 & 98.37 \\
9fc3e@0  & 0.87 & 2.56  & 91.34 & 99.78 \\
598a5@0  & 1.31 & 2.73  & 90.24 & 97.82 \\
1292e@0  & 2.31 & 6.91  & 38.49 & 80.02 \\
817fb@0  & 4.54 & 8.74  & 19.33 & 68.27 \\
e1fa67@0 & 5.54 & 25.58 & 7.98  & 32.93 \\
9bb17@5  & 4.50 & 12.86 & 22.31 & 54.15 \\
cde36@1  & 1.65 & 5.41  & 76.93 & 95.76 \\
\bottomrule
\end{tabular*}
\vspace{-0.9em}
\end{wraptable}


We next evaluate the Future-State Visuomotor Target Predictor independently from the policy. Table~\ref{tab:predictor_eval} reports future-state prediction quality with 3D error in cm, 2D UV error in pixels, and PCK (Percentage of Correct Keypoints) in 5 and 10 pixels. The predictor performs accurately on cutting/stirring tasks, while shearing is more challenging. 
The performance of the target predictor shows a consistent pattern with that of the overall policy. Challenging tasks involve narrow tool-object contact regions, and abrupt motion changes, making future states harder to infer from the observation history alone. The tasks considered for testing are all unseen during training. We provide the full training tasks ID in the \textbf{Supplementary Material}.
%\BL{Either use bold, italic or none. We used bold in the previous reference to supplmenatry material.}

\begin{wraptable}[11]{r}{0.50\linewidth}
\vspace{-1.0em}
\centering
\caption{\textbf{Ablation on future prediction horizon.}
We compare different future horizon schedules.}
\label{tab:horizon_ablation}
\vspace{-0.5em}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Task ID} &
\textbf{3D} $\downarrow$ &
\textbf{UV} $\downarrow$ &
\textbf{PCK@5} $\uparrow$ &
\textbf{PCK@10} $\uparrow$ \\
\midrule
083f7@0\_h24  & 1.66 & 4.05 & 71.87 & 97.54 \\
083f7@0\_h16  & 1.47 & 3.32 & 79.56 & 98.37 \\
083f7@0\_h8   & 1.19 & 3.68 & 76.99 & 96.34 \\
9fc3e@0\_h24  & 1.11 & 2.95 & 86.66 & 99.27 \\
9fc3e@0\_h16  & 0.87 & 2.56 & 91.34 & 99.78 \\
9fc3e@0\_h8   & 0.84 & 2.46 & 92.15 & 99.72 \\
598a5@0\_h24  & 1.77 & 3.97 & 73.56 & 97.46 \\
598a5@0\_h16  & 1.31 & 2.73 & 90.24 & 97.82 \\
598a5@0\_h8   & 1.38 & 2.86 & 89.72 & 97.40 \\
\bottomrule
\end{tabular}}
\vspace{-1.0em}
\end{wraptable}

Table~\ref{tab:horizon_ablation} shows the effect of the receding horizon, which is directly tied to the temporal hierarchy in DexFuture. A short horizon is easier to predict, but provides less future guidance to the controller. A long horizon covers more policy steps, but becomes harder to predict reliably. We choose $h16$ as the default horizon, corresponding to $\{0,2,4,\ldots,16\}$, which provides the best overall trade-off. This supports our hierarchical design that the high-level predictor produces future targets at a slower timescale, while the policy executes dense low-level actions.


\subsection{Qualitative Results}

\begin{figure*}[!t]
  \centering
  \includegraphics[width=\textwidth]{dexfuture/figures/exp_result.pdf}
\caption{\textbf{Qualitative comparison on bimanual dexterous tool-use tasks.}
From top to bottom: 1. chop knife cutting bread (083f7@0). 2. fruite knife cutting apple (9fc3e@0). 3. shear paper with scissors (9bb17@5). 4. wipe whiteboard with brush (fc88d@0). From left to right: 1. ManipTrans with ground-truth target. 2. PhysGraph with ground-truth target 3. PhysGraph without target. 4. Our DexFuture with predicted target. The privileged baselines can access the demonstration targets, while DexFuture infers the future target from visuomotor history alone. The no-target policy fails to maintain robust hand-tool-object interaction, whereas DexFuture recovers stable tool use and produces rollouts comparable to the oracle policies. We include more tasks and full videos in the \textbf{Supplementary Material}.
}
\label{fig:results}
\end{figure*}
%\BL{It would be better if the four rows in Fig 3 all show the same task. At least write which tasks these show in the caption.}

Figure~\ref{fig:results} visualizes representative rollouts. The no-target policy often loses stable hand-tool-object coordination, confirming that current-state feedback alone is insufficient for these tasks. In contrast, DexFuture produces motions that closely follow the oracle target-conditioned policies: the hands maintain tool grasp, approach the object with appropriate alignment, and complete contact-rich interactions such as cutting, wiping, and shearing. These qualitative results complement Table~\ref{tab:policy}, which shows that DexFuture is not simply improving a scalar success metric, but restoring the coordinated structure that target-conditioned dexterous policies rely on. The predicted target acts as a coarse future guidance, while the policy performs the local contact correction for execution.

\subsection{Comparison with Action-Conditioned Planning}
\label{sec:dexwm}
To validate our choice of \emph{action-free} predictor with a policy rather than an \emph{action-conditioned} world model with planning for dexterous tool use, we further compare DexFuture with the strongest action-conditioned dexterous world-model planning baseline following DexWM~\cite{dexwm}. We train the default DexWM model on the EgoDex dataset \cite{egodex}, evaluate on DexWM's default dataset to get comparable results to those reported in \cite{dexwm}, then further evaluate variants with and without finetuning on our OakInk2 tool-use tasks. We test both short and long-horizon planning. The best performance was obtained by finetuning on the OakInk2 dataset, and by using a planning horizon of 1 (next RGB frame as the goal). However, it still underperforms DexFuture. More importantly, testing using the same single 3090Ti GPU, DexWM's default CEM-based planning runs at approximately $0.24$Hz, while DexFuture executes at the policy control rate of $60$Hz. The $250\times$ speed gap is critical for high-DoF dexterous manipulation, where contact-rich actions must be updated at high frequency. These results highlight the practical advantage of our hierarchy: instead of optimizing over counterfactual future action sequences online, DexFuture amortizes future target generation into a low-frequency visuomotor predictor and leaves high-frequency action control to the policy. The full comparison is described in the \textbf{Supplementary Material}. 



==> dexfuture/sec/introduction.tex <==
\section{Introduction}
Bimanual dexterous tool use remains a central challenge in robot learning, requiring two high-DoF hands to coordinate indirect contacts through a tool while interacting with an object. Recent learning-based methods have made impressive progress by leveraging demonstrations as strong guidance for dexterous control. In particular, target-conditioned policies make high-DoF manipulation more tractable by providing the policy with future reference targets extracted from demonstration trajectories ~\cite{dexmachina,dextrack,omnigrasp,maniptrans,physgraph}. These targets can encode future hand motion, object pose, fingertip relations, and task-level cues. However, they are also privileged. At deployment, the robot observes the current scene and proprioception, but does not have access to the future demonstration state. Thus, a key bottleneck is generating a dynamically meaningful future target trajectory without relying on privileged future demonstrations.

A natural alternative is to learn an action-conditioned world model and use online planning to select future actions~\cite{dexwm}. This enables counterfactual rollouts, but requires optimizing over many high-dimensional candidate action sequences at inference. For dexterous tool use, such planning remains computationally prohibitive for the high frequency needed for stable contact-rich control. A plausible compromise is to retain a fast target-conditioned policy and make only the high-level target predictor action-conditioned. However, this exposes a dependency loop: future actions depend on predicted future targets, while the predictor itself would require future actions as input.
%\BL{This makes sense to us, but perhaps not to the reader because we are implicitly assuming that the world model sits on top of the policy. Need to revise.} 
This motivates a different formulation: rather than planning over future actions online, can we predict the future target interface directly from visuomotor history while still preserving the control advantages of future targets?

We propose \textbf{DexFuture}, a hierarchical future-state visuomotor control framework for bimanual dexterous tool use, illustrated in Fig.~\ref{fig:fig1}. DexFuture couples a high-level Future-State Visuomotor Target Predictor with a low-level Target-Conditioned Structured Dexterous Policy. The predictor observes recent egocentric RGB frames and proprioceptive/geometric states, and predicts a coarse future target trajectory over multiple policy steps. The policy then tracks the predicted and interpolated targets at every step to produce high-frequency bimanual actions. This hierarchy separates \emph{what/where} the manipulation should progress toward in the future from \emph{how} to execute contact-rich actions, while also separating slow long-horizon prediction from fast per-step control.

We evaluate DexFuture on challenging bimanual tool-use tasks from OakInk2~\cite{oakink2}, including cutting, pouring, wiping, shearing, and stirring. DexFuture removes the need for privileged future demonstration targets while recovering most of the performance of the oracle target-conditioned policy. Compared with a no-target policy, it substantially improves task success, showing that future targets remain essential for dexterous tool use. Compared with DexWM-style CEM planning \cite{dexwm}, DexFuture executes at the policy control rate, highlighting the practical advantage of amortized target prediction over online action-sequence optimization.

Our contributions are summarized as follows:
\begin{itemize}[leftmargin=1.2em, itemsep=0em, topsep=0em, parsep=0em, partopsep=0em]
\item We propose \textbf{DexFuture}, a hierarchical future-state visuomotor targeting framework that couples a high-level Future-State Visuomotor Target Predictor with a low-level Target-Conditioned Structured Dexterous Policy, separating coarse future-state guidance from high-frequency dexterous action execution.
\item We introduce an action-free future target prediction module that replaces privileged future demonstration targets with predicted targets conditioned on RGB and proprioceptive/geometric history, using structured visuomotor tokenization and sparse multi-horizon target prediction.
\item We validate DexFuture on challenging bimanual dexterous tool-use tasks, showing that predicted targets recover most of the privileged-oracle performance, strongly outperform no-target control, and execute substantially faster than DexWM-style CEM planning.
\end{itemize}

==> dexfuture/sec/related_work.tex <==
\section{Related Work}
\paragraph{Dexterous manipulation from demonstrations and targets.}
Learning dexterous manipulation directly from sparse task rewards is difficult due to the high DOF of hands and contact-rich dynamics. A common strategy is to leverage human demonstrations, retargeted references, or structured future targets to make policy learning tractable~\cite{dexpilot,dexmv,bidexhands,dexpoint,unidexgrasp,dextrack,maniptrans,dexmachina,dexmimicgen,omnigrasp,physgraph}. Large hand-object datasets and egocentric manipulation datasets further provide rich supervision for learning hand trajectories, object interactions, and task structure~\cite{dexycb,arctic,grab,hoi4d,oakink2,egodex}. These works show the importance of demonstration-guided or target-conditioned control, especially for high-DoF dexterous hands. However, the future reference or target used by the policy is often extracted from the demonstration trajectory and contains privileged future hand, tool, or object states that are unavailable at deployment. DexFuture aims to retain the performance of target-conditioned policies, while obviating demonstration targets by \emph{predicting} the future target from visuomotor history.

\paragraph{World models and action-conditioned planning.}
World models learn predictive representations for decision making and have been widely used with model-predictive control and trajectory optimization~\cite{dreamerv3,tdmpc,tdmpc2,mwm,mvmwm}. Recent predictive representation models and video world models further scale future prediction with latent objectives or controllable generative models~\cite{ijepa,vjepa,nwm,dit}. For dexterous manipulation, DexWM~\cite{dexwm} learns an action-conditioned world model from large-scale videos and uses the cross entropy method (CEM) to plan next actions~\cite{cem}. Such action-conditioned models are suitable for counterfactual rollouts, but online planning over high-dimensional dexterous action sequences is expensive and difficult to run at contact-control frequency. Our proposed method, DexFuture, takes a different route: it uses an action-free predictor to generate future-state targets directly, then delegates high-frequency action execution to a target-conditioned policy.

==> sec/abstract.tex <==



\begin{abstract}
Bimanual dexterous tool use remains challenging for robots due to high-dimensional hand configurations and complex hand-tool-object dynamics and contact. 
%Target-conditioned dexterous policies make these tasks tractable by using future targets from demonstrations as input, but the targets contain privileged future hand-tool-object states that are unavailable at deployment. Future action-conditioned world models enable counterfactual planning, but require online optimization over high-dimensional action sequences and are too slow for contact-rich dexterous control. 
%\BL{I would change these two sentences (target-conditioned policies, world model) to something like: A significant challenge is generating a dynamically consistent future reference trajectory without relying on privileged states from demonstrations or slow counterfactual planning. Should talk about our method more, rather than list out previous work.}
Most existing control policies depend on future configuration references provided from demonstrations, while future action-conditioned world models require slow online planning over high-dimensional action sequences.
A significant challenge is generating a dynamically consistent future reference trajectory without relying on privileged states from demonstrations or slow counterfactual planning.
We propose \textbf{DexFuture}, a hierarchical system that couples a high-level \emph{Future-State Visuomotor Target Predictor} with a low-level \emph{Target-Conditioned Structured Dexterous Policy}. Conditioned on egocentric RGB, proprioceptive and geometric history, the high-level predictor constructs structured hand-tool-object visuomotor embeddings and uses a horizon-conditioned transformer to generate a multi-step future target trajectory. 
%\NA{This sentence can mention something about the technical approach for doing so.}. 
Then, the low-level policy tracks them with a target-conditioned per-link transformer. %\NA{This sentence can mention something about the technical approach for doing so.}. 
This hierarchy decouples coarse future reference generation from fine-grained action control, and slow long-horizon semantic prediction from high-frequency execution. On OakInk2 bimanual tool-use tasks, DexFuture achieves $90\%$ of the privileged-oracle performance, compared to $7\%$ for a no-reference policy. DexFuture operates at $60$ Hz, approximately $250\times$ faster than DexWM-style Cross-Entropy Method (CEM)
%\NA{Spell out CEM or even better refer more specifically to DexWM.}
planning with a future action-conditioned world model. Project Website: \url{https://blarklee.github.io/DexFuture_official_website/}
\end{abstract}

% Two or three meaningful keywords should be added here
\keywords{Bimanual Dexterous Tool Use, Visuomotor Future-State Prediction, Target-Conditioned Control}

==> sec/backup.tex <==
Bimanual dexterous tool use remains a formidable challenge in robotics due to high-dimensional hand control, coordinated multi-contact interactions, and complex hand--tool--object dynamics. Recent target-conditioned dexterous policies make such tasks more tractable by tracking future targets extracted from demonstration trajectories. However, these targets contain privileged future hand, tool, and object states, and are unavailable at deployment. Action-conditioned world models provide another route through online planning, but require expensive optimization over high-dimensional future actions, making them impractical for high-frequency contact-rich dexterous control. We propose \textbf{DexFuture}, a hierarchical future-state visuomotor targeting framework that removes the need for privileged future demonstration targets. DexFuture uses a high-level Future-State Visuomotor Target Predictor to infer a coarse multi-step target window from causal egocentric RGB and proprioceptive/geometric history. A low-level target-conditioned structured dexterous policy then tracks the predicted and interpolated targets at every simulator step to execute fast bimanual actions. This hierarchy separates future-state targeting from action-level control, and slow semantic prediction from high-frequency execution. On challenging OakInk2 bimanual tool-use tasks, DexFuture recovers the benefit of target-conditioned control without privileged future targets, achieving $59.69\%$ average success rate compared with $7.36\%$ for the no-target policy and about $90\%$ of the privileged oracle. DexFuture also executes at $60$Hz, approximately $250\times$ faster than CEM-based action-conditioned planning in our setup. Our results show that predicted future-state targets provide an efficient and practical interface between visuomotor perception and dexterous control.




We propose DexFuture, a hierarchical system that couples a high-level Future-State Visuomotor Predictor with a low-level Physically-Grounded Dexterous Policy. The predictor converts RGB observations and proprioception into structured future-state targets, which replace privileged demonstration targets during inference, while the policy executes contact-rich bimanual tool-use manipulation through physically-grounded attention.


DexFuture, A hierarchical visuomotor framework that couples a slow predictive visual target generator with a fast physically-grounded dexterous control policy. .




During DexFuture execution, the same slot is filled with the target predicted by Eq.~\eqref{eq:target_decoder}. This isolates the key question studied in this paper: whether the benefit of target-conditioned dexterous control can be preserved when future targets are inferred from visuomotor history rather than provided by privileged demonstration state.

While the high-level visuomotor predictor predicts coarser guidance, our low-level has the ability to correct the action with the noisy guidance input.

We use artimano hands


\begin{wraptable}[13]{r}{0.50\textwidth}
\vspace{-0.8em}
\centering
\caption{\textbf{Future-state target prediction accuracy.}
We report 3D error, UV error, and PCK within 5/10 pixels.}
\label{tab:predictor_eval}
\vspace{-0.5em}
\footnotesize
\setlength{\tabcolsep}{2pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccc@{}}
\toprule
\textbf{Task ID} &
\textbf{3D} $\downarrow$ &
\textbf{UV} $\downarrow$ &
\textbf{PCK@5} $\uparrow$ &
\textbf{PCK@10} $\uparrow$ \\
\midrule
083f7@0  & 1.47 & 3.32  & 79.56 & 98.37 \\
9fc3e@0  & 0.87 & 2.56  & 91.34 & 99.78 \\
598a5@0  & 1.31 & 2.73  & 90.24 & 97.82 \\
1292e@0  & 2.31 & 6.91  & 38.49 & 80.02 \\
b4a4e@1  & 3.17 & 14.49 & 13.92 & 41.45 \\
817fb@0  & 4.54 & 8.74  & 19.33 & 68.27 \\
e1fa67@0 & 5.54 & 25.58 & 7.98  & 32.93 \\
9bb17@5  & 4.50 & 12.86 & 22.31 & 54.15 \\
cde36@1  & 1.65 & 5.41  & 76.93 & 95.76 \\
\bottomrule
\end{tabular*}
\vspace{-0.9em}
\end{wraptable}


\begin{wraptable}[12]{r}{0.50\linewidth}
\vspace{-1.0em}
\centering
\caption{\textbf{Ablation of future prediction horizon.}
We compare different future horizon schedules using 3D error, UV error, and PCK within 5/10 pixels.}
\label{tab:horizon_ablation}
\vspace{-0.5em}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Task ID} &
\textbf{3D} $\downarrow$ &
\textbf{UV} $\downarrow$ &
\textbf{PCK@5} $\uparrow$ &
\textbf{PCK@10} $\uparrow$ \\
\midrule
083f7@0\_h24  & 1.66 & 4.05 & 71.87 & 97.54 \\
083f7@0\_h16  & 1.47 & 3.32 & 79.56 & 98.37 \\
083f7@0\_h8   & 1.19 & 3.68 & 76.99 & 96.34 \\
9fc3e@0\_h24  & 1.11 & 2.95 & 86.66 & 99.27 \\
9fc3e@0\_h16  & 0.87 & 2.56 & 91.34 & 99.78 \\
9fc3e@0\_h8   & 0.84 & 2.46 & 92.15 & 99.72 \\
598a5@0\_h24  & 1.77 & 3.97 & 73.56 & 97.46 \\
598a5@0\_h16  & 1.31 & 2.73 & 90.24 & 97.82 \\
598a5@0\_h8   & 1.38 & 2.86 & 89.72 & 97.40 \\
\bottomrule
\end{tabular}}
\vspace{-1.0em}
\end{wraptable}



\iffalse
\begin{table}[htbp]
\centering
\begin{minipage}{0.5\linewidth}
\centering
\caption{\textbf{Quantitative results on bimanual tool-use tasks of Oakink2 dataset \cite{oakink2}.} Link 3D Error (cm), Percentage of correct key points, Link UV Error (pix), link\_pck\_5px (\%), link\_pck\_10px (\%)}
\label{table:physgraph_results}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Task ID}  & \textbf{3D} $\uparrow$ & \textbf{UV} $\downarrow$ & \textbf{pck\_5px} $\uparrow$ & \textbf{pck\_10px} $\uparrow$ \\ 
\midrule
{083f7@0\_h24}   & 1.66 & 4.05 & 71.87 & 97.54 \\
{083f7@0\_h16}   & 1.47 & 3.32 & 79.56 & 98.37 \\
{083f7@0\_h8}   & 1.19 & 3.68 & 76.99 & 96.34 \\
{9fc3e@0\_h24}   & 1.11 & 2.95 & 86.66 & 99.27 \\
{9fc3e@0\_h16}   & 0.87 & 2.56 & 91.34 & 99.78 \\
{9fc3e@0\_h8}   & 0.84 & 2.46 & 92.15 & 99.72  \\
{598a5@0\_h24}  & 1.77 & 3.97 & 73.56 & 97.46 \\
{598a5@0\_h16}  & 1.31 & 2.73 & 90.24 & 97.82 \\
{598a5@0\_h8}  & 1.38 & 2.86 & 89.72 & 97.40 \\
\bottomrule
\end{tabular}
\label{tab:horizon_ablation}
}
\end{minipage}
\end{table}
\fi

==> sec/limitation.tex <==
\section{Limitations and Future Work}
\label{sec:limitations}
The main remaining bottleneck is future target prediction under difficult contacts. Tasks with narrow contact regions or abrupt tool motion remain challenging. The high-level predictor must be robust enough to guide the precise action of low-level policy. Potential future solutions should focus on uncertainty-aware or contact-aware prediction, stronger visual grounding under occlusion, and deployment to a real robot.
%\BL{I would change the last item to "deployment to a real robot."}


